Analyzing the "Sleeping Giants" Activism Model in Brazil

In 2020, amidst the COVID pandemic and a polarized political climate, the Sleeping Giants online activist movement gained traction in Brazil. Its rationale was simple: to curb the spread of misinformation by harming the advertising revenue of sources that produce this type of content. Like its international counterparts, Sleeping Giants Brasil (SGB) campaigned against media outlets using Twitter to ask companies to remove ads from the targeted outlets. This work presents a thorough quantitative characterization of this activism model, analyzing the three campaigns carried out by SGB between May and September 2020. To do so, we use digital traces from both Twitter and Google Trends, toxicity and sentiment classifiers trained for the Portuguese language, and an annotated corpus of SGB's tweets. Our key findings were threefold. First, we found that SGB's requests to companies were largely successful (with 83.85\% of all 192 targeted companies responding positively) and that user pressure was correlated to the speed of companies' responses. Second, there were no significant changes in the online attention and the user engagement going towards the targeted media outlets in the six months that followed SGB's campaign (as measured by Google Trends and Twitter engagement). Third, we observed that user interactions with companies changed only transiently, even if the companies did not respond to SGB's request. Overall, our results paint a nuanced portrait of internet activism. On the one hand, they suggest that SGB was successful in getting companies to boycott specific media outlets, which may have harmed their advertisement revenue stream. On the other hand, they also suggest that the activist movement did not impact the online attention these media outlets received nor the online image of companies that did not respond positively to their requests.

==> Makefile <==
title = main
latex  = pdflatex 
papers = $(title).tex

all: pdf

pdf : $(papers)
	$(latex) $(papers)
	bibtex $(title)
	perl -pi -e 's/\{10\}/\{10\}\n\\vspace\{0.2cm\}/gi' $(title).bbl
	$(latex) $(papers)
	$(latex) $(papers)

clean:
	rm -rf $(title).bbl $(title).blg $(title).log $(title).out $(title).aux

abstract.txt: sections/abstract.tex
	cat $< |grep -v '\\begin' | grep -v '\\end' | \
	    sed -e '/^%/d' | \
	    sed -e 's/\\sys/$(SYS)/g' | \
	    sed -e 's/~/ /g' | \
	    sed -e 's/{//g' | \
	    sed -e 's/}//g' | \
	    sed -e 's/\\%/%/g' | \
	    fmt -w72 > $@


==> images/fix_dict.tex <==
    \begin{tabular}{p{0.2\linewidth}|p{0.7\linewidth}}
\toprule
Incels & 
female(s)
normie(s)
chad(s)
virgin
whore(s)
girl(s)
rope
gf
girlfriend
women
whore
beta
cunt
suicide
pussy
woman
bitches
cuck(s)
bitch
feminism \\ \midrule
T\_D & 
trans
commie
dem(s)
democrat(s)
deep
communist
diversity
leftist
communism
antifa
socialist
left
socialism
libs
gender\\ \bottomrule
\end{tabular}

